Signal Subspace Methods Which Are Robust to Impulsive Noise

We consider the problem of estimating a signal subspace in the presence of interference that contaminates some proportion of the received observations. Our emphasis is on detecting the contaminated observations so that the signal subspace can be estimated with the contaminated observations discarded. To this end, we employ a signal model which explicitly includes an interference term that is distinct from environmental noise. To detect when the interference term is nonzero, we estimate the interference term using an optimization problem with a sparsity-inducing group SLOPE penalty which accounts for simultaneous sparsity across all channels of the multichannel signal. We propose an iterative algorithm which efficiently computes the observations estimated to contain interference. Theoretical support for the accuracy of our interference estimator is provided by bounding its false discovery rate, the expected proportion of uncontaminated observations among those estimated to be contaminated. Finally, we demonstrate the empirical performance of our contributions in a number of simulated experiments.

==> thebib.tex <==

@article{brzyski2019group,
  title={Group slope--adaptive selection of groups of predictors},
  author={Brzyski, Damian and Gossmann, Alexej and Su, Weijie and Bogdan, Ma{\l}gorzata},
  journal={Journal of the American Statistical Association},
  volume={114},
  number={525},
  pages={419--433},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{henderson1986impulse,
  title={Impulse noise: critical review},
  author={Henderson, D and Hamernik, RP},
  journal={The Journal of the Acoustical Society of America},
  volume={80},
  number={2},
  pages={569--584},
  year={1986},
  publisher={Acoustical Society of America}
}

@article{schmidt1981signal,
  title={A signal subspace approach to multiple emitter location and spectral estimation},
  author={Schmidt, RO},
  journal={Ph. D. thesis, Stanford University},
  year={1981}
}

@techreport{abramovich1999impulsive,
  title={Impulsive noise mitigation in spatial and temporal domains for surface-wave over-the-horizon radar},
  author={Abramovich, Yuri I and Turcaj, Pavel},
  year={1999},
  institution={COOPERATIVE RESEARCH CENTRE FOR SENSOR SIGNAL AND INFORMATION PROCESSING~…}
}

@book{etter2018underwater,
  title={Underwater acoustic modeling and simulation},
  author={Etter, Paul C},
  year={2018},
  publisher={CRC press}
}

@article{middleton1999non,
  title={Non-Gaussian noise models in signal processing for telecommunications: new methods an results for class A and class B noise models},
  author={Middleton, David},
  journal={IEEE Transactions on Information Theory},
  volume={45},
  number={4},
  pages={1129--1149},
  year={1999},
  publisher={IEEE}
}

@article{davis1997adaptive,
  title={Adaptive greedy approximations},
  author={Davis, Geoff and Mallat, Stephane and Avellaneda, Marco},
  journal={Constructive approximation},
  volume={13},
  number={1},
  pages={57--98},
  year={1997},
  publisher={Springer}
}

@book{wainwright2019high,
  title={High-dimensional statistics: A non-asymptotic viewpoint},
  author={Wainwright, Martin J},
  volume={48},
  year={2019},
  publisher={Cambridge University Press}
}

@article{yuan2006model,
  title={Model selection and estimation in regression with grouped variables},
  author={Yuan, Ming and Lin, Yi},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={68},
  number={1},
  pages={49--67},
  year={2006},
  publisher={Wiley Online Library}
}

@article{zou2006adaptive,
  title={The adaptive lasso and its oracle properties},
  author={Zou, Hui},
  journal={Journal of the American statistical association},
  volume={101},
  number={476},
  pages={1418--1429},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={Wiley Online Library}
}

@article{bogdan2015slope,
  title={SLOPE—adaptive variable selection via convex optimization},
  author={Bogdan, Ma{\l}gorzata and Van Den Berg, Ewout and Sabatti, Chiara and Su, Weijie and Cand{\`e}s, Emmanuel J},
  journal={The annals of applied statistics},
  volume={9},
  number={3},
  pages={1103},
  year={2015},
  publisher={NIH Public Access}
}

@article{belloni2011square,
  title={Square-root lasso: pivotal recovery of sparse signals via conic programming},
  author={Belloni, Alexandre and Chernozhukov, Victor and Wang, Lie},
  journal={Biometrika},
  volume={98},
  number={4},
  pages={791--806},
  year={2011},
  publisher={Oxford University Press}
}

@article{zou2005regularization,
  title={Regularization and variable selection via the elastic net},
  author={Zou, Hui and Hastie, Trevor},
  journal={Journal of the royal statistical society: series B (statistical methodology)},
  volume={67},
  number={2},
  pages={301--320},
  year={2005},
  publisher={Wiley Online Library}
}

@article{paulraj,
  title={16 subspace methods for directions-of-arrival estimation},
  author={Paulraj, Arogyaswami and Ottersten, Bj{\"o}rn and Roy, R and Swindlehurst, A and Xu, Guanghan and Kailath, Thomas},
  journal={Handbook of Statistics},
  volume={10},
  pages={693--739},
  year={1993},
  publisher={Elsevier}
}

@article{zoubir2012robust,
  title={Robust estimation in signal processing: A tutorial-style treatment of fundamental concepts},
  author={Zoubir, Abdelhak M and Koivunen, Visa and Chakhchoukh, Yacine and Muma, Michael},
  journal={IEEE Signal Processing Magazine},
  volume={29},
  number={4},
  pages={61--80},
  year={2012},
  publisher={IEEE}
}

@article{rousseeuw1984least,
  title={Least median of squares regression},
  author={Rousseeuw, Peter J},
  journal={Journal of the American statistical association},
  volume={79},
  number={388},
  pages={871--880},
  year={1984},
  publisher={Taylor \& Francis}
}

@article{visuri2001subspace,
  title={Subspace-based direction-of-arrival estimation using nonparametric statistics},
  author={Visuri, Samuli and Oja, Hannu and Koivunen, Visa},
  journal={IEEE Transactions on Signal Processing},
  volume={49},
  number={9},
  pages={2060--2073},
  year={2001},
  publisher={IEEE}
}

@article{oja1997robust,
  title={Robust covariance matrix estimation with signal processing applications},
  author={Oja, H and Koivunen, V},
  journal={The Yerbook of the Finnish Statistical Society},
  pages={87--109},
  year={1997}
}

@article{huber1981robust,
  title={Robust statistics},
  author={Huber, Peter J},
  journal={Wiley Series in Probability and Mathematical Statistics},
  year={1981}
}

@inproceedings{gossmann2015identification,
  title={Identification of significant genetic variants via SLOPE, and its extension to group SLOPE},
  author={Gossmann, Alexej and Cao, Shaolong and Wang, Yu-Ping},
  booktitle={Proceedings of the 6th ACM Conference on Bioinformatics, Computational Biology and Health Informatics},
  pages={232--240},
  year={2015}
}

@book{golub2013matrix,
  title={Matrix computations},
  author={Golub, Gene H and Van Loan, Charles F},
  year={2013},
  publisher={JHU press}
}

@article{grippo2000convergence,
  title={On the convergence of the block nonlinear Gauss--Seidel method under convex constraints},
  author={Grippo, Luigi and Sciandrone, Marco},
  journal={Operations research letters},
  volume={26},
  number={3},
  pages={127--136},
  year={2000},
  publisher={Elsevier}
}

@book{efron2021computer,
  title={Computer Age Statistical Inference: Algorithms, Evidence, and Data Science},
  author={Efron, Bradley and Hastie, Trevor},
  volume={6},
  year={2021},
  publisher={Cambridge University Press}
}

@article{goodman1963statistical,
  title={Statistical analysis based on a certain multivariate complex Gaussian distribution (an introduction)},
  author={Goodman, Nathaniel R},
  journal={The Annals of mathematical statistics},
  volume={34},
  number={1},
  pages={152--177},
  year={1963},
  publisher={JSTOR}
}

@book{rossing2007springer,
  title={Springer Handbook of Acoustics},
  author={Rossing, Thomas},
  year={2007},
  publisher={Springer Science \& Business Media}
}

@article{cadzow1988high,
  title={A high resolution direction-of-arrival algorithm for narrow-band coherent and incoherent sources},
  author={Cadzow, James A},
  journal={IEEE Transactions on Acoustics, Speech, and Signal Processing},
  volume={36},
  number={7},
  pages={965--979},
  year={1988},
  publisher={IEEE}
}

@article{parikh2014proximal,
  title={Proximal algorithms},
  author={Parikh, Neal and Boyd, Stephen and others},
  journal={Foundations and trends{\textregistered} in Optimization},
  volume={1},
  number={3},
  pages={127--239},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{mirsky1975trace,
  title={A trace inequality of John von Neumann},
  author={Mirsky, Leon},
  journal={Monatshefte f{\"u}r mathematik},
  volume={79},
  pages={303--306},
  year={1975},
  publisher={Springer}
}

@misc{oh-thesis,
	year = {2022-12},
	author = {Oh, Micah Y.},
	keywords = {acoustic, underwater, signal, interference, slope, regression, noise, simulation, sparsity},
	publisher = {Monterey, CA; Naval Postgraduate School},
	title = {Robstifying Signal Subspace Methods with Group SLOPE},
}

